A HoTT Quantum Equational Theory (Extended Version)

This paper presents an equational theory for the QRAM model of quantum computation, formulated as an embedded language inside of homotopy type theory. The embedded language approach is highly expressive, and reflects the style of state-of-the art quantum languages like Quipper and QWIRE. The embedding takes advantage of features of homotopy type theory to encode unitary transformations as higher inductive paths, simplifying the presentation of an equational theory. We prove that this equational theory is sound and complete with respect to established models of quantum computation.

==> cc.tex <==
A term context, informally, is a term with holes in it.
\begin{align*}
        C ∷=~&□ ∣ \letin{x}{C}{e'} ∣ \letin{x}{e}{C} \\
          &∣ (C,e₂) ∣ (e₁,C) \\
          &∣ \letin{(x,y)}{C}{e'} ∣ \letin{(x,y)}{e}{C} \\
          &∣ ι₀ C ∣ ι₁ C \\
          &∣ \caseof{C}{ι₀ x₀ → e₀}{ι₁ x₁ → e₁} \\
          &∣ \caseof{e}{ι₀ x₀ → C₀}{ι₁ x₁ → C₁} \\
          &∣ C >! f ∣ e >! λ x.C
\end{align*}
In this section we make this notion more formal.

The type of term contexts, written $\TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Γ'}{r}$, is indexed by two components.
\begin{itemize}

\item $\vect{(αᵢ;Γᵢ)} :\List{(\Type × \Ctx)}$ correspond to the holes of the
  term context, which will be filled with arguments of type $αᵢ → Γᵢ,Δ ⊢ - : q$;

  \item after filling the holes with arguments of the correct type, the
    resulting expression will have type $Δ,Γ' ⊢ - : r$.
\end{itemize}

Term contexts are defined inductively as in \cref{fig:TCtx}.


\begin{figure}
{ \small
\[ \begin{array}{c}
    \inferrule*
    {~}
    {□ : \TCtx{[((),·)]}{q}{·}{q}}
  \\ \\
    \inferrule*
    { C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Γ'}{r} \\
      Δ',x:r ⊢ e' : s }
    { \letin{x}{C}{e'} : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ',Γ'}{s} }
  \qquad
    \inferrule*
    { Δ ⊢ e : r \\
      C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Γ',x:r}{s} }
    { \letin{x}{e}{C} : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ,Γ'}{s} }
  \\ \\
    \inferrule*
    { C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ₁}{r₁} \\
      Δ₂ ⊢ e₂ : r₂ }
    { (C,e₂) : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ₁,Δ₂}{r₁ ⊗ r₂} }
  \qquad
    \inferrule*
    { C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ₁}{r₁} \\
      Δ₂ ⊢ e₂ : r₂ }
    { (C,e₂) : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ₁,Δ₂}{r₁ ⊗ r₂} }
  \\ \\
    \inferrule*
    { C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ}{r₁ ⊗ r₂} \\
      Δ',x₁:r₁,x₂:r₂ ⊢ e' : s }
    { \letin{(x₁,x₂)}{C}{e'} : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ,Δ'}{s} }
  \\ \\
    \inferrule*
    { Δ ⊢ e : r₁ ⊗ r₂ \\
      C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ',x₁:r₁,x₂:r₂}{s} }
    { \letin{(x₁,x₂)}{e}{C} : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ,Δ'}{s} }
  \\ \\
    \inferrule*
    { C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ}{r₀} }
    { ι₀ C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ}{r₀ ⊕ r₁} }
  \qquad
    \inferrule*
    { C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ}{r₁} }
    { ι₁ C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ}{r₀ ⊕ r₁} }
  \\ \\
    \inferrule*
    { C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ}{r₀ ⊕ r₁} \\
      Δ',x₀ : r₀ ⊢ e₀ : s \\
      Δ',x₁ : r₁ ⊢ e₁ : s }
    { \caseof{C}{ι₀ x₀ → e₀}{ι₁ x₁ → e₁} : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ,Δ'}{s} }
  \\ \\
    \inferrule*
    { Δ ⊢ e : r₀ ⊕ r₁ \\
      C₀ : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ',x₀:r₀}{s}  \\
      C₁ : \TCtx{\vect{(βⱼ;Δⱼ)}}{q}{Δ',x₁:r₁}{s} }
    { \caseof{e}{ι₀ x₀ → C₀}{ι₁ x₁ → C₁} :
                \TCtx{\vect{(αᵢ;Γᵢ)},\vect{(βⱼ;Δⱼ)}}{q}{Δ,Δ'}{s} }
  \\ \\
    \inferrule*
    { C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ}{\Lower{β}} \\
      f : β → Δ' ⊢ - : r }
    { C >! f : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ,Δ'}{r} }
  \\ \\
    \inferrule*
    { Δ ⊢ e : \Lower{β} \\
      C : β → \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Δ'}{r} }
    { e >! C : \TCtx{\vect{(β → αᵢ;Γᵢ)}}{q}{Δ,Δ'}{r} }
\end{array} \] }
\caption{Term Contexts}
\label{fig:TCtx}
\end{figure}


\begin{lemma}
  For any term context $C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Γ}{r}$, context $Δ$, and
  paramaterized terms $tᵢ : αᵢ → Γᵢ,Δ ⊢ - : q$, there is a term
  $Γ,Δ ⊢ C[\vect{tᵢ}] : r$.
\end{lemma}
\begin{proof}
  Straightforward by induction on $C$.
\end{proof}

\begin{lemma}
  For term contexts $C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Γ}{r}$ and
  $D : \TCtx{\vect{(βⱼ;Δⱼ)}}{r}{Δ}{s}$, there is a term context
  $D ∘ C : \TCtx{\vect{(αᵢ × βⱼ; Γᵢ,Δⱼ)}}{q}{Γ,Δ}{s}$ such that
  \[
    D ∘ C[t_{i,j}]
    = D\left[\vect{λ (b : βⱼ). 
      C\left[\vect{λ (a : αᵢ).t_{i,j}(a,b)}\right]}\right]
  \]
\end{lemma}
\begin{proof}
  By induction on $C$.
\end{proof}

\begin{definition}
  An \emph{elimination context} is a term context whose holes occur in the
  rightmost position of an elimination form:
  \begin{align*}
        E ∷=~&□ ∣ \letin{x}{e}{C} \\
          &∣ \letin{(x,y)}{e}{C} \\
          &∣ \caseof{e}{ι₀ x₀ → C₀}{ι₁ x₁ → C₁} \\
          &∣ e >! λ x.C
  \end{align*}
  Formally, the holes of elimination contexts can be filled terms of any type,
  and the result will have the same form. An elimination context
  $\ECtx{\vect{(αᵢ;Γᵢ)}}{Γ'}$ is defined as in \cref{fig:ECtx}.
\end{definition}



\begin{figure}
\[ \begin{array}{c}
    \inferrule*
    {~}
    {□ : \ECtx{[((),·)]}{·}}
  \\ \\
    \inferrule*
    { Δ ⊢ e : r \\
      C : \ECtx{\vect{(αᵢ;Γᵢ)}}{Γ',x:r} }
    { \letin{x}{e}{C} : \ECtx{\vect{(αᵢ;Γᵢ)}}{Δ,Γ'} }
  \\ \\
    \inferrule*
    { Δ ⊢ e : r₁ ⊗ r₂ \\
      C : \ECtx{\vect{(αᵢ;Γᵢ)}}{Δ',x₁:r₁,x₂:r₂} }
    { \letin{(x₁,x₂)}{e}{C} : \ECtx{\vect{(αᵢ;Γᵢ)}}{Δ,Δ'} }
  \\ \\
    \inferrule*
    { Δ ⊢ e : r₀ ⊕ r₁ \\
      C₀ : \ECtx{\vect{(αᵢ;Γᵢ)}}{Δ',x₀:r₀}  \\
      C₁ : \ECtx{\vect{(βⱼ;Δⱼ)}}{Δ',x₁:r₁} }
    { \caseof{e}{ι₀ x₀ → C₀}{ι₁ x₁ → C₁} :
                \ECtx{\vect{(αᵢ;Γᵢ)},\vect{(βⱼ;Δⱼ)}}{Δ,Δ'} }
  \\ \\
    \inferrule*
    { Δ ⊢ e : \Lower{β} \\
      C : β → \ECtx{\vect{(αᵢ;Γᵢ)}}{Δ'} }
    { e >! C : \ECtx{\vect{(β → αᵢ;Γᵢ)}}{Δ,Δ'} }
\end{array} \]
\caption{Elimination Contexts}
\label{fig:ECtx}
\end{figure}


\begin{lemma}
  For any elimination context $E : \ECtx{\vect{(αᵢ;Γᵢ)}}{Γ}$ and quantum type
  $q$, there is a term context $E^q : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Γ}{q}$.
\end{lemma}

\begin{axiom}[Commuting conversions]
  Let $C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Γ}{r}$ be a term context and let
  $E : \ECtx{\vect{(βⱼ;Δⱼ)}}{Δ}$ be an elimination context. Then
  \[
    C ∘ E^q[\vect{t_{i,j}}] ∼_{cc} E^r ∘ C[\vect{t_{i,j}}].
  \]
\end{axiom}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



==> equations.tex <==
Beyond the $β$ and $η$ rules for the linear type system given in the previous
section, we introduce additional rules to the equational theory that describe
how unitary transformations relate to other constructs, inspired by~\citet{staton2015}.
These rules come in two forms:

First, we consider a number of structural rules.
\begin{align}
    \unitary{U}{e} &= \unitary{V}{e} \quad\text{if } U=V \\
    \unitary{(U₁ ⊗ U₂)}{(e₁,e₂)} &= (\unitary{U₁}{e₁}, \unitary{U₂}{e₂}) \\
    \unitary{(U₀ ⊕ U₁)}{(ι₀ e)} &= \unitary{U₀}{e} \\
    \unitary{(U₀ ⊕ U₁)}{(ι₁ e)} &= \unitary{U₁}{e} \\
    \unitary{U}{(\unitary{V}{e})} &= \unitary{(U ∘ V)}{e} \\
    \unitary{I}{e} &= e \\
    \unitary{U}{(\letin{()}{e}{e'})} &= \letin{()}{e}{\unitary{U}{e'}} \\
    \unitary{U}{(\letin{(x₁,x₂)}{e}{e'})} &= \letin{(x₁,x₂)}{e}{\unitary{U}{e'}} \\
    \unitary{U}{(\caseof{e}{ι₀ x₀ → e₀}{ι₁ x₁ → e₁})}
        &= \caseof{e}{ι₀ x₀ → \unitary{U}{e₀}}
                     {ι₁ x₁ → \unitary{U}{e₁}} \\
    \unitary{U}{(e >! f)} &= e >! λ x → \unitary{U}{(f x)} \\
    \meas{(\unitary{U}{e})} >! λ \_ → e' &= \meas{e} >! λ \_ → e'
\end{align}
\jennifer{What is the status of η equivalence?}


In addition, there are a number of semantic relationships between specific
unitaries and their elements. For example, for the ``not'' unitary
transformation $X$ swaps the value of basis elements and the results of
measurement:
\begin{align*}
    \texttt{X} (\new{b}) &= \new{¬ b} \\
    \meas{(\texttt{X} e)} &= \letin{!x}{\meas{e}}{\put{¬x}}
\end{align*}
For the ``controlled-not'' unitary $CNOT$, which operates on two qubits, its
behavior is described as followed:
\begin{Coq}
    CNOT (new b, e) = (new b, if b then X e else e)

    let (x,y) = CNOT (e₁,e₂) in
    let !_    = meas x       in e'
  = let !b    = meas e₁      in
    let y     = if b then X e₂ else e₂ in e'
\end{Coq}

These types of equations can thus be broken up into two parts:
\begin{enumerate}
    \item The relationship between the unitary and initialization, and
    \item The relationship between the unitary and measurement.
\end{enumerate}

In a later section we will characterize these as two stand-alone axioms. 



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> semantics-proofs.tex <==
In this section we prove that the equational theory is sound with respect to the
denotational semantics (\cref{thm:hott:soundness}) by proving the soundness of each
of the component relations: $∼_β$, $~_{cc}$, and $~_q$. 

We start with the observation that the padding $s$ in $⟦e⟧^s$ is the identity on
that part of the quantum state. 

\begin{lemma} \label{lem:hott:pad-commute} %
  If $Γ ⊢ e : q$ and $A : \Matrix(α,β)$, then
  \[
        ⟦e⟧^{\point{β}} ∘ (I ⊗ A)^* = (I ⊗ A)^* ∘ ⟦e⟧^{\point{α}}.
  \]

  In addition,
  \[
     \DISTR^* ∘ ⟦e⟧^{(r₀ ⊕ r₁) ⊗ s} = (⟦e⟧^{r₀ ⊗ s} ⊕ ⟦e⟧^{r₁ ⊗ s}) ∘ \DISTR.
  \]

  Furthermore, if $Γ ⊢ e : q$ and $Γ' ⊢ e' : q'$ where $Γ$ and $Γ'$ are
  disjoint, then 
  \[ ⟦e⟧^{q'⊗ s} ∘ ⟦e'⟧^{Γ ⊗ s} = ⟦e'⟧^{q ⊗ s} ∘ ⟦e'⟧^{Γ' ⊗ s}. \]
\end{lemma}



To prove that $β$ equivalence is sound in this semantics, we must first prove a
substitution lemma. For a substitution $σ ≡ \{eᵢ / xᵢ\}$ where $Γᵢ ⊢ eᵢ : qᵢ$
for $1 ≤ i ≤ n$, we write $⟦σ⟧^s : ⟦Γ₁ ⊗ ⋯ ⊗ Γₙ ⊗ s⟧ → ⟦q₁ ⊗ ⋯ ⊗ qₙ ⊗ s⟧$ for
$⟦(e₁,…,eₙ)⟧^s$.


\begin{lemma} \label{lem:hott:substitution-sound}
    If $Γᵢ ⊢ eᵢ : qᵢ$ and $Γ',x₁:q₁,…,xₙ:qₙ ⊢ e' : r$, then 
    $⟦e'\{eᵢ/xᵢ\}⟧$ is equal to
    \[ \begin{tikzcd}
        ⟦ Γ₁ ⊗ Γ₂ ⊗ ⋯ ⊗ Γₙ ⊗ Γ' ⟧
            \arrow[rr,"⟦(e₁ … eₙ)⟧^{Γ'}"] & &
        ⟦ q₁ ⊗ q₂ ⊗ ⋯ ⊗ qₙ ⊗ Γ' ⟧
            \arrow[r,"⟦e'⟧"] &
        ⟦ r ⟧
    \end{tikzcd} \]
\end{lemma}
\begin{proof}
    By induction on $e'$. We will expand upon a few illustrative cases.

    \begin{enumerate}[-]

    \item
    Consider $e' ≡ \letin{y}{d}{d'}$, where $Γ'≡Δ,Δ'$ such that
    $Δ,x₁:q₁,…,xₖ:qₖ ⊢ d : s$ and $Δ',x_{k+1}:q_{k+1},…,xₙ:qₙ ⊢ d' : r$. Then we
    have
    \begin{align*}
      ⟦e'\{eᵢ/xᵢ\}⟧ &≡ ⟦ \letin{y}{d\{e₁,…,eₖ/x₁,…,xₖ\}}
                                  {d'\{e_{k+1},…,eₙ/x_{k+1},…,xₙ\}}⟧ \\
        &≡ ⟦d'\{e_{k+1},…,eₙ/x_{k+1},…,xₙ\}⟧ 
         ∘ ⟦d\{e₁,…,eₖ/x₁,…,xₖ\}⟧^{Δ',Γ_{k+1},…,Γₙ} \\
        &= ⟦d'⟧ ∘ ⟦(e_{k+1},…,e_n)⟧^{r,Δ'} 
        ∘ ⟦d⟧^{Δ',Γ_{k+1},…,Γₙ} ∘ ⟦(e₁,…,eₖ)⟧^{Δ,Δ',Γ_{k+1},…,Γₙ}
        & \text{(Induction Hypothesis)} \\
        &= ⟦d'⟧ ∘ ⟦d⟧^{Δ',q_{k+1},…,qₙ} 
         ∘ ⟦(e_{k+1},…,eₙ)⟧^{Δ,Δ'} ∘ ⟦(e₁,…,e_k)⟧^{Δ,Δ',Γ_{k+1},…,Γₙ}
        & \text{(\cref{lem:hott:pad-commute})} \\
        &≡ ⟦\letin{y}{d}{d'}⟧ ∘ ⟦(e₁,…,eₙ)⟧^{Δ,Δ'}
    \end{align*}

  \item Consider $e' ≡ d ⸖ f$ where $Γ'≡Δ,Δ'$ such that
    $Δ,x₁:q₁,…,xₖ:qₖ ⊢ d : \Lower{α}$ and
    $f : α → Δ',x_{k+1}:q_{k+1},…,xₙ:qₙ ⊢ - : r$. Then:
    \begin{align*}
        ⟦e'\{eᵢ/xᵢ\}⟧ 
        &≡ ⟦d\{e₁,…,eₖ/x₁,…,xₖ\} ⸖ λ a. f a \{e_{k+1},…,eₙ/x_{k+1},…,xₙ\}⟧ \\
        &≡ \sum_{a : α} ⟦f a \{e_{k+1},…,eₙ/x_{k+1},…,xₙ\}⟧ ∘ (δ_a^† ⊗ I)^* 
                      ∘ ⟦d\{e₁,…,eₖ/x₁,…,xₖ\}⟧^{Δ',Γ_{k+1},…,Γₙ} \\
        &= \sum_{a : α} ⟦f a⟧ ∘ ⟦(e_{k+1},…,eₙ)⟧^{Δ'} ∘ (δ_a^† ⊗ I)^* 
                      ∘ ⟦d⟧^{Δ',Γ_{k+1},…,Γₙ} ∘ ⟦(e₁,…,eₖ)⟧^{Δ,Δ',Γ_{k+1},…,Γₙ} 
            & \text{(IH)} \\
        &= \sum_{a : α} ⟦f a⟧ ∘ (δ_a^† ⊗ I)^* ∘ ⟦d⟧^{Δ',q_{k+1},…,qₙ} 
                      ∘ ⟦(e_{k+1},…,eₙ)⟧^{Δ,Δ'} ∘ ⟦(e₁,…,eₖ)⟧^{Δ,Δ',Γ_{k+1},…,Γₙ}
            & \text{(\cref{lem:hott:pad-commute})} \\
        &≡ ⟦d ⸖ f⟧ ∘ ⟦(e₁,…,eₙ)⟧^{Δ,Δ'}
    \end{align*}

    \end{enumerate}
    The remaining cases are similar.
\end{proof}


\begin{theorem}[Soundness of $β$-equivalence]
    If $e₁ ∼_β e₂$ then $⟦e₁⟧ = ⟦e₂⟧$.
\end{theorem}
\begin{proof}
  For the $β$ rules for $\letin{x}{e}{e'}$ and $\letin{(x₁,x₂)}{(e₁,e₂)}{e'}$,
  the result follows directly from \cref{lem:hott:substitution-sound}. 
  \begin{enumerate}[-]

  \item Consider
  \[
     \caseof{ιᵢ e}{ι₀ x₀ → e₀}{ι₁ x₁ → e₁} ∼_β eᵢ\{e / xᵢ\}.
  \]
  For the denotations of the two terms to be equal, it suffices to check that
  $(f₀ ⊕ f₁)(ιᵢ^\ast(ρ)) = fᵢ(ρ)$. Notice
  \begin{align*}
    (f₀ ⊕ f₁)(ιᵢ^\ast(ρ)) \quad≡\quad (f₀ ⊕ f₁)(ιᵢ ρ ιᵢ^†)
    \quad≡\quad f₀ (ι₀^† ιᵢ ρ ιᵢ^† ι₀) + f₁ (ι₁^† ιᵢ ρ ιᵢ^† ι₁)
  \end{align*}
  When $i ≠ j$ we have $ιⱼ^† ιᵢ = 0$, and when $i = j$ we have $ιⱼ^† ιᵢ = I$;
  thus the expression reduces to $fᵢ(ρ)$.


  \item Consider 
  \[ 
    \put{a} ⸖ f ∼_β f a.
  \]
  Expanding out definitions, we see that
  \begin{align*}
    ⟦ \put{a} ⸖ f ⟧(ρ) \quad≡\quad \sum_{a}⟦f a⟧ ∘ (δ_a^†)^* ∘ δ_a^* (ρ)
        \quad=\quad \sum_{a}⟦f a⟧ ∘ (δ_a^† δ_a)^* (ρ).
  \end{align*}
  Again, we have $δ_{aᵢ}^† δₐ ≡ I$ if $a = aᵢ$, and $0$ otherwise, so the
  right-hand-side of this expression reduces to $⟦f a⟧(ρ)$.
  \end{enumerate}
\end{proof}



% To prove the soundness of commuting conversions, we can prove that the denotation of a commuting conversion can be factored out into its constituent parts.

% \begin{lemma} \label{lem:hott:cc-denote} For any
%   $C : \TCtx{\vect{(αᵢ;Γᵢ)}}{q}{Γ'}{r}$, there is a superoperator
%   $\overline{C} : ⟦q⟧ → ⟦r⟧$, as well as a collection of superoperators
%   $\underline{C}_i^s : ⟦Γ' ⊗ s⟧ → ⟦Γᵢ ⊗ s⟧$ such that for
%   $tᵢ : αᵢ → Γᵢ,Δ ⊢ - : q$, we have
%   \[
%     ⟦C[\vect{tᵢ}]⟧ = \sum_i \sum_{a : αᵢ} \overline{C} ∘ ⟦tᵢ a⟧ ∘ \underline{C}_i^Δ.
%   \]
% \end{lemma}
% \begin{proof}
% \jennifer{todo}
% \end{proof}

To demonstrate the soundness of commuting conversions, we consider one case at a
time.

\begin{lemma} \label{lem:hott:cc-denote}
    Let $C$ be a term context. Then
  \begin{align}
    ⟦C[\letin{x}{e}{e'}]⟧ 
%        &= ⟦\letin{x}{e}{C[e']}⟧ 
        &≡ ⟦C[e']⟧ ∘ ⟦e⟧ 
            \label{eqn:hott:letin-cc} \\
    ⟦C[\letin{(x₁,x₂)}{e}{e'}]⟧ 
%        &= ⟦\letin{(x₁,x₂)}{e}{C[e']}⟧  
        &≡ ⟦C[e']⟧ ∘ ⟦e⟧ 
            \label{eqn:hott:letpair-cc} \\
    ⟦C[\caseof{e}{ι₀ x₀ → e₀}{ι₁ x₁ → e₁}]⟧
%        &= ⟦ \caseof{e}{ι₀ x₀ → C[e₀]}{ι₁ x₁ → C[e₁]} ⟧
        &≡ (⟦C[e₀]⟧ ⊕ ⟦C[e₁]⟧) ∘ \DISTR ∘ ⟦e⟧ 
            \label{eqn:hott:caseof-cc}\\
    ⟦C[e ⸖ f]⟧ 
%        &= ⟦e ⸖ λ a.~C[f a]⟧
        &≡ \sum_a ⟦C[f a]⟧ ∘ (δ_a^† ⊗ I) ∘ ⟦e⟧
            \label{eqn:hott:letbang-cc}
  \end{align}
\end{lemma}
\begin{proof}
  By induction on $C$. Here we will consider a representative sample of
  cases.
  \begin{enumerate}

  \item Consider $C ≡ (C₁,e₂)$ where $Δ₂ ⊢ e₂ : q₂$ and consider
    $C[\caseof{e}{ι₀ x₀ → e₀}{ι₁ x₁ → e₁}]$ where $Δ ⊢ e : r₀ ⊕ r₁$ and
    $Δ',xᵢ:rᵢ ⊢ eᵢ : q$.
    Then the left-hand-side of \cref{eqn:hott:caseof-cc} is equal to
        $⟦(C₁[\caseof{e}{ι₀ x₀ → e₀}{ι₁ x₁ → e₁}],e₂)⟧$
    which, by the inductive hypothesis, expands out to
    \begin{align*}
        ⟦Δ ⊗ Δ' ⊗ Γ₁ ⊗ Γ₂⟧
            &\xrightarrow{⟦e₂⟧^{Δ,Δ',Γ₁}}
        &&⟦Δ ⊗ Δ' ⊗ Γ₁ ⊗ q₂⟧ \\
            &\xrightarrow{⟦e⟧^{Δ',Γ₁,q₂}}
        &&⟦(r₀ ⊕ r₁) ⊗ Δ' ⊗ Γ₁ ⊗ q₂⟧  \\
            &\xrightarrow{\DISTR}
        &&⟦(r₀ ⊗ Δ' ⊗ Γ₁ ⊗ q₂) ⊕ (r₁ ⊗ Δ' ⊗ Γ₁ ⊗ q₂)⟧ \\
            &\xrightarrow{⟦C₁[e₀]⟧ ⊕ ⟦C₁[e₁]⟧}
        &&⟦q₁ ⊗ q₂⟧
    \end{align*}
  By \cref{lem:hott:pad-commute}, this is equal to 
    \begin{align*}
        ⟦Δ ⊗ Δ' ⊗ Γ₁ ⊗ Γ₂⟧
            &\xrightarrow{⟦e⟧^{Δ',Γ₁,Γ₂}}
        &&⟦(r₀ ⊕ r₁) ⊗ Δ' ⊗ Γ₁ ⊗ Γ₂⟧  \\
            &\xrightarrow{\DISTR}
        &&⟦(r₀ ⊗ Δ' ⊗ Γ₁ ⊗ Γ₂) ⊕ (r₁ ⊗ Δ' ⊗ Γ₁ ⊗ Γ₂)⟧ \\
            &\xrightarrow{⟦e₂⟧⊕ ⟦e₂⟧}
        &&⟦(r₀ ⊗ Δ' ⊗ Γ₁ ⊗ q₂) ⊕ (r₁ ⊗ Δ' ⊗ Γ₁ ⊗ q₂)⟧ \\
            &\xrightarrow{⟦C₁[e₀]⟧ ⊕ ⟦C₁[e₁]⟧}
        &&⟦q₁ ⊗ q₂⟧
    \end{align*}
    But 
    \[ 
        (⟦C₁[e₀]⟧ ⊕ ⟦C₁[e₁]⟧) ∘ (⟦e₂⟧ ⊕ ⟦e₂⟧) 
      = (⟦C₁[e₀]⟧ ∘ ⟦e₂⟧) ⊕ (⟦C₁[e₁]⟧ ∘ ⟦e₂⟧)
      = ⟦(C₁[e₀],e₂)⟧ ⊕ ⟦(C₁[e₁],e₂)⟧,
    \]
    which completes the proof of this case.



\item Consider $C ≡ \letin{(y₁,y₂)}{C'}{e'}$ where the goal is to show that 
\[ ⟦C[e ⸖ f] ⟧ = \sum_a ⟦C[f a]⟧ ∘ (δₐ^† ⊗ I)^* ∘ ⟦e⟧.
\]
    Expanding out the left-hand-side, we get
    \begin{align*}
        ⟦\letin{(y₁,y₂)}{C'[e ⸖ f]}{e'}⟧
        &≡ ⟦e'⟧ ∘ ⟦C'[e ⸖ f]⟧  \\
        &= ⟦e'⟧ ∘ \sum_a ⟦C'[f a]⟧ ∘ (δₐ^† ⊗ I)^* ∘ ⟦e⟧
        \qquad\text{(Induction Hypothesis)} \\
        &= \sum_a ⟦e'⟧ ∘ ⟦C'[f a]⟧ ∘ (δₐ^† ⊗ I)^* ∘ ⟦e⟧ \\
        &≡ \sum_a ⟦ \letin{(y₁,y₂)}{e'}{C'[f a]}⟧ ∘ (δₐ^† ⊗ I)^* ∘ ⟦e⟧.
    \end{align*}

\item Consider $C ≡ e' ⸖ C'$. Then
    \begin{align*}
        ⟦C[\caseof{e}{ι₀ x₀ → e₀}{ι₁ x₁ → e₁}]⟧
        &≡ \sum_a ⟦C' a [\caseof{e}{ι₀ x₀ → e₀}{ι₁ x₁ → e₁}]⟧ 
             ∘ (δ_a^† ⊗ I)^* ∘ ⟦e'⟧ \\
        &= \sum_a (⟦C' a[e₀]⟧ ⊕ ⟦C' a[e₁]⟧) ∘ \DISTR ∘ ⟦e⟧
             ∘ (δ_a^† ⊗ I)^* ∘ ⟦e'⟧ 
    \end{align*}
    by the inductive hypothesis. By \cref{lem:hott:pad-commute} we can commute these around each other to obtain
    \begin{align*}
        &\sum_a (⟦C' a[e₀]⟧ ⊕ ⟦C' a[e₁]⟧) 
              ∘ \left((δ_a^† ⊗ I)^* ⊕ (δ_a^† ⊗ I)^*\right)
              ∘ (⟦e'⟧ ⊕ ⟦e'⟧)
              ∘ \DISTR ∘ ⟦e⟧ \\
        &=
         \left(\sum_a \left(⟦C' a[e₀]⟧ \circ (δ_a^† ⊗ I)^* ∘ ⟦e'⟧ \right) 
              ⊕ \sum_a \left(⟦C' a[e₁]⟧ \circ (δ_a^† ⊗ I)^* ∘ ⟦e'⟧ \right) 
         \right)
              ∘ \DISTR ∘ ⟦e⟧ \\
        &≡ \left(⟦e ⸖ λ a.~C' a[e₀]⟧ ⊕ ⟦e ⸖ λ a.~C' a[e₁]⟧\right)
              ∘ \DISTR ∘ ⟦e⟧ 
    \end{align*}
  \end{enumerate}
\end{proof}



\begin{theorem}[Soundness of commuting conversions]
   For any term context $E$ and evaluation context $C$,
  \[
      ⟦C ∘ E^q[\vect{tᵢ}]⟧ = ⟦E^r ∘ C[\vect{tᵢ}]⟧.
  \]
\end{theorem}
\begin{proof}
  By induction on $E$, using \cref{lem:hott:cc-denote}.
\end{proof}





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

